The ins and outs of iteration in Mezzo

This is a talk proposal for HOPE 2013. Using iteration over a collection as a case study, we wish to illustrate the strengths and weaknesses of the prototype programming language Mezzo.

==> Makefile <==
# ----------------------------------------------------------------------------
# Set any paper-specific variables.

include Makefile.local

# ----------------------------------------------------------------------------
# Eliminate the default known suffixes.

.SUFFIXES:

# ----------------------------------------------------------------------------
# Definitions.

LATEX    := pdflatex --shell-escape
PROLOGUE := \def\fppdf{true}\nonstopmode\input

# ----------------------------------------------------------------------------
# Generic rules.

%.pdf: *.tex *.sty ../common/*.tex ../common/*.bib *.mz *.mzi
	$(LATEX) "$(PROLOGUE)" $(DOC).tex
	bibtex $(DOC)
	$(LATEX) "$(PROLOGUE)" $(DOC).tex
	$(LATEX) "$(PROLOGUE)" $(DOC).tex

# ----------------------------------------------------------------------------
# Targets.

.PHONY: pdf clean export

pdf: $(DOC).pdf

clean::
	rm -f *.aux *.log *.bbl *.blg *~ *.out *.thm
	rm -f $(DOC).dvi $(DOC).pdf

# ----------------------------------------------------------------------------
# Web export.

WWW   := yquem.inria.fr:public_html/publis
SHORT := gueneau-pottier-protzenko-iteration-in-mezzo.pdf

export: pdf
	scp -p -B -C $(DOC).pdf $(WWW)/$(SHORT)


==> courte-ou-longue.tex <==
\makeatletter
\IfFileExists{switch.tex}{
  \input{switch.tex}
  \@ifundefined{fplong}{
  \newenvironment{courte}{}{}
  \newenvironment{longue}{\comment}{\endcomment}
  }{
  \@ifundefined{WhizzyTeX}{\usepackage[pdftex]{changebar}}{\usepackage[dvips]{changebar}}
  \newenvironment{courte}{\comment}{\endcomment}
  \newenvironment{longue}{}{}
  }
}{}
\makeatother


==> figure-fifo.tex <==
\begin{figure}[t]
\begin{lstlisting}[numbers=left]
data mutable cell a =
  Cell { elem: a; next: dynamic } -- \label{line:next:dynamic}

data mutable bag a =
     Empty { head, tail: () }
| NonEmpty { head, tail: dynamic } -- \label{line:head-tail:dynamic}
adopts cell a -- \label{line:adopts}

val create [a] () : bag a =
  Empty { head = (); tail = () }

val insert [a] (consumes x: a, b: bag a) : () =
  let c = Cell { elem = x; next = () } in
  c.next <- c;
  give c to b; -- \label{line:adopt}
  match b with -- \label{line:match:one}
  | Empty ->
      tag of b <- NonEmpty; -- \label{line:empty-to-nonempty:begin}
      b.head <- c; -- \label{fig:write:c:1}
      b.tail <- c -- \label{line:empty-to-nonempty:end} \label{fig:write:c:2}
  | NonEmpty ->
      take b.tail from b; -- \label{line:focus:entry}
      b.tail.next <- c; -- \label{fig:write:c:3}
      give b.tail to b; -- \label{line:focus:exit}
      b.tail <- c -- \label{fig:write:c:4}
  end

val retrieve [a] (b: bag a) : option a =
  match b with -- \label{line:match:two}
  | Empty ->
      None
  | NonEmpty ->
      take b.head from b; -- \label{line:abandon}
      let x = b.head.elem in -- \label{line:head:elem}
      if b.head == b.tail then begin
        tag of b <- Empty; -- \label{line:nonempty-to-empty:begin}
        b.head <- ();
        b.tail <- () -- \label{line:nonempty-to-empty:end}
      end else begin
        b.head <- b.head.next -- \label{line:head:next}
      end;
      Some { value = x }
  end
\end{lstlisting}
\caption{A FIFO implementation of bags}
\label{fig:fifo}
\end{figure}


==> macros.tex <==
\makeatletter

\newcommand{\mezzo}{%
  \texorpdfstring{%
    \protect\mbox{%
      \protect\textit{\protect\textsf{%
        Me\protect\raisebox{-.1ex}z\protect\hspace{-.3ex}{\protect\raisebox{.2ex}z}\protect\hspace{-.1ex}o%
      }}%
    }%
  }{Mezzo}\xspace
}

\newcommand{\hamlet}{\mezzo}
\newcommand{\ocaml}{OCaml\xspace}

\@ifpackageloaded{listings}{
  \lstset{
    language=caml,
    flexiblecolumns=false,
    showstringspaces=false,
    basicstyle=\tt\small,
    framesep=5pt,
    numberstyle=\tiny,
    numbersep=5pt,
    escapeinside={--}{\^^M},
    morekeywords={data,val,consumes,adopts,take,give,from},
  }
  \def\li{\lstinline}
  \def\qli|#1|{``\li|#1|''}
  \def\sqli|#1|{``\texttt{\small #1}''}

}

\@ifpackageloaded{tikz}{

  \newcommand{\inlinetikzbox}[2]{%
    \tikz[baseline]{%
      \node[fill=gray!20,anchor=base] (#1) {#2};%
    }%
  }

  \AtBeginDocument{\tikzstyle{every picture}+=[remember picture]}
}{}



\@ifpackageloaded{color}{
  \definecolor{mygrey}{rgb}{0.9,0.9,0.9}
  \newcommand{\mystrut}{\rule[-.1\baselineskip]{0pt}{.65\baselineskip}}
  \newcommand{\shaded}[1]{\colorbox{mygrey}{$\mystrut\smash{#1}$}}
}{}

\makeatother


\newcommand{\kw}[1]{\ensuremath{\text{\textsf{#1}}}}
\newcommand{\ktype}{\ensuremath{\kw{type}}}
\newcommand{\kterm}{\kw{term}}
\newcommand{\kperm}{\kw{perm}}

\newcommand{\kreset}{\kw{extend}}
\newcommand{\kleft}{\kw{left}}
\newcommand{\kright}{\kw{right}}
\newcommand{\khead}{\kw{head}}
\newcommand{\ktail}{\kw{tail}}
\newcommand{\ktrue}{\kw{true}}
\newcommand{\kfalse}{\kw{false}}

\newcommand{\kconsumes}{\kw{consumes}}

\makeatletter
\@ifundefined{mode}{
  \newcommand{\mode}[1]{\ensuremath{m\,#1}}
}{}
\makeatother

\newcommand{\moded}{\kw{duplicable}}
\newcommand{\modex}{\kw{exclusive}}
\newcommand{\modea}{\kw{affine}}

\newcommand{\fhead}{\kw{head}}
\newcommand{\ftail}{\kw{tail}}
\newcommand{\nret}{\kw{ret}}

\newcommand{\tyvar}                   {a} % variable of kind type
\newcommand{\tyunknown}               {\kw{unknown}}
\newcommand{\tydynamic}               {\kw{dynamic}}
\newcommand{\tydynamicprime}[1]       {\kw{dynamic}'\,#1}
\newcommand{\tyarrow}[2]              {\ensuremath{#1 \rightarrow #2}}
\newcommand{\tyearrow}[2]              {\ensuremath{#1 \rightsquigarrow #2}}
\newcommand{\tytuple}[1]              {\ensuremath{(#1)}}
\newcommand{\tyconcretezero}[1]   {\ensuremath{\kw{#1}}}
\newcommand{\tyconcrete}[2]   {\ensuremath{\kw{#1}\,\{ #2 \}}}
\newcommand{\tyconcretev}[2]   {\ensuremath{\vec{\kw{#1}}\,\{ #2 \}}}
\newcommand{\tyconcreteadopts}[3]   {\ensuremath{\kw{#1}\,\{ #2 \}\,\kw{adopts}\,#3}}
\newcommand{\tyapp}[2]                {\ensuremath{#1\ #2}}
\newcommand{\tynameintro}[2]          {\ensuremath{#1: #2}}
\newcommand{\tyconsumes}[1]           {\ensuremath{\kw{consumes}\ #1}}
\newcommand{\tyforall}[3]             {\ensuremath{\forall(#1: #2)\ #3}}
\newcommand{\tyexists}[3]             {\ensuremath{\exists(#1: #2)\ #3}}
\newcommand{\tyforalln}[2]            {\ensuremath{[#1]\;#2}}
\newcommand{\tybar}[2]                {\ensuremath{(#1\mid#2)}}
\newcommand{\tysingleton}[1]{\raisebox{0.0mm}{\mbox{\kw{=}}}#1}
\newcommand{\tyand}[2]                {\tybar{#1}{#2}}
\newcommand{\tyimplies}[2]            {\ensuremath{#1 \Rightarrow #2}}
\newcommand{\tyempty}                 {\kw{empty}}
\newcommand{\tystar}[2]               {\ensuremath{#1 \ast #2}}
\newcommand{\tyatomic}[2] {\ensuremath{#1\,@\ #2}}

\newcommand{\tyint}                   {\kw{int}}
\newcommand{\tystring}                {\kw{string}}
\newcommand{\tyref}[1]                {\kw{ref}\;#1}
\newcommand{\tylist}[1]               {\kw{list}\;#1}
\newcommand{\tymlist}[1]              {\kw{mlist}\;#1}
\newcommand{\tymtree}[1]              {\kw{mtree}\;#1}
\newcommand{\typackage}[2]            {\tybar{\tysingleton{#1}}{\tyatomic{#1}{#2}}}

\newcommand{\econstraint}[2]          {\ensuremath{#1\!: #2}}
\newcommand{\equalified}[2]           {\ensuremath{#1\!\!::\!\!#2}}
\newcommand{\elet}[3]                 {\ensuremath{\kw{let}\ #1=#2\ \kw{in}\ #3}}
\newcommand{\efun}[3]                 {\ensuremath{\kw{fun}\ #1:#2=#3}}
\newcommand{\elambda}[4]              {\ensuremath{\lambda(#1:#2)\!: #3.\ #4}}
\newcommand{\eLambda}[3]              {\ensuremath{\Lambda(#1:#2).\ #3}}
\newcommand{\eassign}[3]              {\ensuremath{#1.#2 \leftarrow #3}}
\newcommand{\eassigntag}[2]           {\ensuremath{\kw{tag of}\ #1 \leftarrow \kw{#2}}}
\newcommand{\eaccess}[2]              {\ensuremath{#1.#2}}
\newcommand{\eassert}[1]              {\ensuremath{\kw{assert}\ #1}}
\newcommand{\eapply}[2]               {\ensuremath{#1\ #2}}
\newcommand{\etapply}[2]              {\ensuremath{#1\ [#2]}}
\newcommand{\ematch}[2]               {\ensuremath{\kw{match}\ #1\ \kw{with}\ #2}}
\newcommand{\pbranch}[2]              {\ensuremath{\,|\ #1 \rightarrow #2}}
\newcommand{\etuple}[1]               {\ensuremath{(#1)}}
\newcommand{\econstruct}[2]           {\ensuremath{\kw{#1}\,\{ #2 \}}}
\newcommand{\eifthenelse}[3]          {\ensuremath{\kw{if}\ #1\ \kw{then}\ #2\ \kw{else}\ #3}}
\newcommand{\esequence}[2]            {\ensuremath{#1;\ #2}}
\newcommand{\egive}[2]                {\ensuremath{\kw{give}\ #1\ \kw{to}\ #2}}
\newcommand{\etake}[2]                {\ensuremath{\kw{take}\ #1\ \kw{from}\ #2}}
\newcommand{\eowns}[2]                {\ensuremath{#1\ \kw{owns}\ #2}}
\newcommand{\efail}                   {\kw{fail}}


\newcommand{\subsub}{\equiv} % we could also use \lessgtr
\newcommand{\tynest}[2]{#1\prec#2}
\newcommand{\tylock}[1]{\kw{lock}\;#1}

\newcommand{\vdashw}{\vdash_\vartriangleright}
\newcommand{\vdashb}{\vdash_\blacktriangleright}

\newcommand{\modeD}[1]{\ensuremath{#1\text{ is duplicable}}}
\newcommand{\modeX}[1]{\ensuremath{#1\text{ is exclusive}}}
\newcommand{\modeA}[1]{\ensuremath{#1\text{ is affine}}}

\newcommand{\kmodeD}{\kw{duplicable}}
\newcommand{\kmodeX}{\kw{exclusive}}
\newcommand{\kmodeA}{\kw{affine}}

\newcommand{\osf}{\multimap} % from amssymb
\def\etal.{\emph{et al.}}


==> pygmentize.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.64,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.94,0.16,0.16}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@l\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.64,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.81,0.36,0.00}{##1}}}
\expandafter\def\csname PY@tok@ld\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.96,0.47,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.77,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.36,0.21,0.80}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.80,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@py\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.20,0.40,0.64}{##1}}}
\expandafter\def\csname PY@tok@x\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.81,0.36,0.00}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@g\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.64,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.81}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@n\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@p\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\let\PY@ul=\underline\def\PY@tc##1{\textcolor[rgb]{0.97,0.97,0.97}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.13,0.29,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.31,0.60,0.02}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.56,0.35,0.01}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


